On transitions in water wave propagation through consolidated to broken sea ice covers

A theoretical model is used to study water waves propagating into and through a region containing thin floating ice, for ice covers transitioning from consolidated (large floe sizes) to fully broken (small floe sizes). The degree of breaking is simulated by a mean floe length. It is shown that there are deterministic limits for consolidated and fully broken ice covers where the wave fields do not depend on the particular realisation of the ice cover for a given mean floe length. The consolidated ice limit is consistent with classic flexural-gravity wave theory, and the fully broken limit is well modelled by Bloch waves in a periodic ice cover. In the transition between the limits, the wave field depends on the ice cover realisation, as multiple wave scattering is a dominant process. The effects of the ice cover on the wave field are quantified using a wavelength, attenuation rate, and a transferred amplitude measuring the amplitude drop at the ice edge. It is shown that as the ice cover breaks up (mean floe size gets smaller), the wavelength and amplitude drop decreases (transferred amplitude increases) and the attenuation rate increases. The results provide a new interpretation of field observations.

==> boxes-luke.tex <==
%% BOXES

\usepackage{tcolorbox}% http://ctan.org/pkg/tcolorbox
\definecolor{mycolor}{rgb}{0.122, 0.435, 0.698}% Rule colour
\makeatletter
\newcommand{\tbox}[5]{
\setbox0=\hbox{#1}%
\setlength{\@tempdima}{\dimexpr\wd0+13pt}%
\begin{tcolorbox}[colback=#3,colframe=#4,
      boxrule=#5,arc=4pt,
      left=6pt,right=6pt,top=6pt,bottom=6pt,boxsep=0pt,
      width=#2]   %\@tempdima]
    #1
\end{tcolorbox}}
\makeatother

\NewDocumentCommand\mybox{om}{%
\IfNoValueTF{#1}{
\tbox{#2}{\textwidth}{white}{mycolor}{2pt}
}{
\tbox{#2}{#1}{white}{mycolor}{2pt}
}}

%\NewDocumentCommand\mytitlebox{om}{%
%\IfNoValueTF{#1}{
%\tbox{#2}{\textwidth}{gray!30}{mycolor}{0pt}
%}{
%\tbox{#2}{#1}{gray!30}{mycolor}{0pt}
%}}
%
%\NewDocumentCommand\myparbox{om}{%
%\IfNoValueTF{#1}{
%\tbox{#2}{\textwidth}{blue!10}{white}{0pt}
%}{
%\tbox{#2}{#1}{blue!10!white!90}{white}{0pt}
%}}
